Homomorphisms and Minimality for Enrich-by-Need Security Analysis

Cryptographic protocols are used in different environments, but existing methods for protocol analysis focus only on the protocols, without being sensitive to assumptions about their environments. LPA is a tool which analyzes protocols in context. LPA uses two programs, cooperating with each other: CPSA, a well-known system for protocol analysis, and Razor, a model-finder based on SMT technology. Our analysis follows the enrich-by-need paradigm, in which models of protocol execution are generated and examined. The choice of which models to generate is important, and we motivate and evaluate LPA's strategy of building minimal models. "Minimality" can be defined with respect to either of two preorders, namely the homomorphism preorder and the embedding preorder (i.e. the preorder of injective homomorphisms); we discuss the merits of each. Our main technical contributions are algorithms for building homomorphism-minimal models and for generating a set-of-support for the models of a theory, in each case by scripting interactions with an SMT solver.

==> evaluation.tex <==
\subsection{Evaluation}\label{sec:evaluation}

% We present the various implemented algorithms for finding minimal
% models and then present performance results.  The first algorithm is
% called the enumerated types (ET) algorithm.

% \begin{algo}[Enumerated Types]\label{alg:et}
%   \noindent
%   \begin{flushleft}
%     Input: theory $T$, output: set of minimal models.
%   \end{flushleft}

%   \vskip1ex
%   \noindent $\cn{ET}(T){}\equiv{}$
%   \begin{listalg}
%   \item $\mM\gets\cn{ET\_first}(T)$.
%   \item If $T$ is unsatisfiable, return.
%   \item $\mN\gets\cn{ET\_last}(T,\seq{\mM})$.
%   \item Output $\mN$.
%   \item $T'\gets T\cup\cn{avoid\_cone}(\mN)$.
%   \item $\cn{ET}(T')$.
%   \end{listalg}

%   \vskip2ex
%   \noindent $\cn{ET\_first}(T\typ\mbox{theory})\typ
%   \mbox{model or \cnc{UNSAT}}{}\equiv{}$
%   \begin{listalg}
%   \item If $T$ is unsatisfiable, return \cnc{UNSAT}.
%   \item Extract domain~$D$ from prover.
%   \item Replace the uninterpreted sorts in~$T$ with enumerated types
%     to form theory~$T'$.  The domain~$D$ is used to determine the
%     number of scalar constants within each enumerated type.
%   \item Ensure $T'$ is satisfiable.
%   \item $\mM\gets\cn{get\_model}(T')$.
%   \item Return $\cn{ET\_min}(T',\mM)$.
%   \end{listalg}

%   \vskip2ex
%   \noindent $\cn{ET\_min}(T\typ\mbox{theory},
%   \mM\typ\mbox{model})\typ\mbox{model}{}\equiv{}$
%   \begin{listalg}
%   \item $T'\gets T\cup{}$ reduction axioms of~$\mM$.
%   \item If $T'$ is unsatisfiable, return~$\mM$.
%   \item $\mN\gets\cn{get\_model}(T')$.
%   \item Return $\cn{ET\_min}(T,\mN)$.
%   \end{listalg}

%   \vskip2ex
%   \noindent $\cn{ET\_last}(T\typ\mbox{theory},
%   M\typ\mbox{sequence of models})\typ\mbox{model}{}\equiv{}$
%   \begin{listalg}
%   \item $T'\gets T\cup\{\cn{avoid\_cone}(\mM)\mid\mM\in M\}$.
%   \item $\mN\gets\cn{ET\_first}(T')$.
%   \item If $T'$ is unsatisfiable, return $\cn{head}(M)$.
%   \item $N\gets{}$ filter out of $M$ models with a homomorphism from~$\mN$.
%   \item Return $\cn{ET\_last}(T,\seq{\mN}\append N)$.
%   \end{listalg}
% \end{algo}

% The \cn{avoid\_cone} function returns the avoid cone associated with a
% simplified version of the model.  Simplification is crucial for
% performance reasons.

% \[\avoid{\mM} \eqdef \neg \homFrom{\mM}\]

%%\subsubsection{Results}

The results of running our test suite is presented in
Table~\ref{tbl:results}.\marginpar{We need betters names for algs.}
John's razor (Algorithm~\ref{alg:et}) is
called ET for Enumerated Types, and
Dan's razor (Algorithm~\ref{alg:us}) is
called US for Uninterpreted Sorts.  The first column names the test.
The columns for each algorithm give the user CPU time in seconds and
the number of satisfaction checks use to obtain an models.  Some of
the tests involve finding models for more than one theory.  The column
contains the number of satisfaction checked used to find models for
each theory encountered in the problem.

\begin{table}
  \begin{center}
  \begin{tabular}{|l|rc|rc|}\hline
    \multicolumn{1}{|c}{Test}&\multicolumn{2}{|c|}{ET}
    &\multicolumn{2}{|c|}{US}\\ \cline{2-5}
    \multicolumn{1}{|c|}{Name}&Time&Sat Cks&Time&Sat Cks\\ \hline
    ../prots/ns/noint&1.67&14 14&1.67&8 7\\
    ../prots/ns/init&1.43&34 12&1.26&9 8\\
    ../prots/reflect/noresp&2.82&11 32&1.89&6 9\\
    ../prots/reflect/resp&1.45&10 30&0.56&5 7\\
    ../prots/doorsep/door&4.32&26 60 37&4.92&9 10 24\\
    1sas/doorsep-no&54.21&123&1.65&11\\
    1sas/doorsep-so&3.41&69&1.10&9\\
    1sas/ns-no&1.38&13&0.99&7\\
    1sas/ns-so&0.48&11&0.56&6\\
    1sas/reflect-so&0.97&30&0.65&8\\
    doorsep-no&11.63&109&1.86&12\\
    doorsep-so&4.54&37&1.10&9\\ \hline
  \end{tabular}
  \end{center}
  \caption{Results}\label{tbl:results}
\end{table}

The results show a clear advantage for UT over ET\@.  UT found models
faster than ET in all but one case.  Furthermore, for the
1sas/doorsep-no test, ET takes about 32 times longer!

UT consistently requested a smaller number of satisfaction checks.
Given the difference, it is surprising ET was competitive at all.

There are some mysteries in the results.  1sas/doorsep-no is the same
as doorsep-no except that the trust rule has been commented out.  With
this causes such a big performance difference is one.  Another mystery
it takes ET longer to solve doorsep-so than ../prots/doorsep/door, the
last problem solved by the latter is doorsep-so!  Something is fishy.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "a-min"
%%% End:

